On the relation of the frame-related operators of fusion frame systems

Frames have been investigated frequently over the last few decades due to their valuable properties, which are desirable for various applications as well as interesting for theory. Some applications additionally require distributed processing techniques, which naturally leads to the concept of fusion frames and fusion frame systems. The latter consists of a system of subspaces, equipped with local frames on each of them, and a global frame. In this paper, we investigate the relations of the associated frame-related operators on all those three levels. For that we provide a detailed investigation on bounded block diagonal operators between Hilbert direct sums. We give the relation of the frame-related operators of the fusion frame and the corresponding frame systems in terms of operator identities. By applying these identities we prove further properties of fusion frame systems.

==> header_xxl.tex <==
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{enumerate}
\usepackage[ansinew]{inputenc}
%\usepackage{times}
%%\usepackage{fixltx2e}
%
\usepackage{hyperref}
\usepackage{multirow}
\usepackage{color}
\usepackage{colortbl}   

\usepackage{wrapfig}
\usepackage{floatflt,epsfig} 
%\usepackage[top=20mm, bottom=20mm, left=20mm, right=20mm]{geometry}
\usepackage{fancyhdr}
\usepackage{array}
\usepackage[right]{eurosym}


% XXL:------------------------------------------------
%\newtheorem{theorem}{Theorem}
\newtheorem{def.}{Definition}
\newtheorem{prop.}[theorem]{Proposition}
\newtheorem{lem.}[theorem]{Lemma}
\newtheorem{cor.}[theorem]{Corollary}
\newtheorem{conj.}[theorem]{Conjecture}
%\newtheorem{example}{Example}
\newtheorem{question}{Question}

%% norm
\newcommand{\norm}[2]{
\left\| #2 \right\|_{#1}
}
\newcommand{\ip}[2]{ \langle {#1} ,{#2}  \rangle}
\newcommand{\ud}{\,\mathrm{d}}

%% Cal:
\def\Hil{\mathcal{H}}
\def\FF{\mathcal{F}}
\def\VV{\mathcal{V}} 
\def\WW{{\mathcal W}}
\def\II{\mathcal{I}}

\def\cD{{\mathcal D}}
\def\cM{{\mathcal M}}
\def\cV{{\mathcal V}}
\def\cN{{\mathcal N}}
\def\cK{{\mathcal K}}
\def\cJ{{\mathcal J}}
\def\cA{{\mathcal A}}
\def\cX{{\mathcal X}}
\def\cI{{\mathcal I}}

%% BB
\def\RR{\mathbb{R}}
\def\ZZ{\mathbb{Z}}
\def\NN{\mathbb{N}}
\def\CC{\mathbb{C}}
\def\EE{\mathbb{E}}
\def\TT{\mathbb{T}}
\def\VV{\mathbb{V}}
\def\QQ{\mathbb{Q}}

\def\RRt{\RR^2}
\def\RRd{\RR^d}
\def\CCd{\CC^d}
\def\TTd{\TT^d}
\def\RRtd{\RR^{2d}}

\def\Bsp{{\boldsymbol B}}   %B-space (boldsymbol)
\def\BspP{{\boldsymbol B'}}   %B'-space (boldsymbol)

\def\Ssp{{\boldsymbol S}}
\def\SOsp{{\Ssp_{\negthinspace 0}}}   %S0-space
\def\SOPsp{{\SOsp{\negthinspace }'}}   %S_0' space (S0-prime space)

%% frac
\def\Af{\mathfrak{A}}
\def\Kf{\mathfrak{K}}
\def\Bf{\mathfrak{B}}
\def\Mf{\mathfrak{M}}
\def\Lf{\mathfrak{L}}

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\ben{\begin{eqnarray}}
\def\een{\end{eqnarray}}


\newcommand{\diag}[1]{
{\mathfrak{diag}} \left( #1 \right)
}


%% direct sums
\newcommand{\ltfun}[2]{\sum \limits_{#1} \bigoplus #2}
\def\ltiv{\ltfun{i\in I}{V_i}}
\def\ltiw{\ltfun{i\in I}{W_i}}

%% Function Spaces
\def\LtR{L^2\left(\RR\right)}
\def\LtRt{L^2\left(\RRt \right)}
\def\LtRd{L^2\left(\RRd \right)}
\def\LtRtd{L^2\left(\RRtd \right)}
\def\Ltwoab{{L^{2} \left(\GG, da d\frac{b}{a^2}\right)}}

\def\LoR{L^1\left(\RR\right)}

\def\llmp{\ell_w^p}

\def\Htwo{H^2(\RR )}

\def\VVmp{V_w^p (\varphi)}

\def\IIo{\left[0,1\right)}
\def\LtIo{L^2\left(\IIo\right)}

\def\IId{\left[0,1\right)^d}
\def\LtId{L^2\left(\IId\right)}

\def\Coosp{{\boldsymbol{\mathcal Co}}}
%\def\Ysp{{\boldsymbol Y}}
\newcommand{\Coo}[1]{{\Coosp \left( #1\right)}}

\def\Oosp{{\boldsymbol{\mathcal O}}}
\newcommand{\Oo}[1]{{\Oosp \left( #1\right)}}

%% Bold 
\def\MM{{\mathbf M}} 
\def\DD{{\mathbf D}}
\def\mm{{\mathbf m}}
\def\GG{{\mathbb G}}


%% bounded linear operators:
\newcommand{\BL}[1]{
{\mathcal B} \left( #1 \right)
}
% \def\BL{\mathfrak B}
\def\HS{{\mathcal HS}}
\def\Sp{{\mathcal S}_p}
\def\Sone{{\mathcal S}_1}
\def\Sq{{\mathcal S}_q}

%% Matrix
\newcommand{\Mat}[1]{
{\mathcal M} \left( #1 \right) 
}
\newcommand{\Matt}[2]{
{\mathcal M}^{\left( #1 \right)} \left( #2 \right) 
}
\newcommand{\Op}[1]{
{\mathcal O}^{\left( #1 \right)} }
\newcommand{\Opp}[2]{
{\mathcal O}^{\left( #1 \right)}\left( #2 \right) }
% empty
%% Matrix
\def\Mate{\mathcal M}
\def\Ope{\mathcal O}


\newcommand{\Hmat}[3]{ \mathcal{M}_{\Hil,#1} \left( #2, #3 \right)}
\def\Hmats{\Hmat{k}{I \times I}{P_2}}


\def\STX{{$ST^X$}}

\def\bds{\limits_{-\infty}^\infty}
\def\bdspos{\limits_{0}^\infty}

\def\inv{{^{-1}}}

%% localiter
%% Banach Algebras
\def\AAa{{\mathcal A}}
\def\AAaa{{\mathcal A}^{(a)}}
\def\BB{{\mathcal B}}
% associated Banach spaces
\def\HHmp{{{\mathcal H}_w^p}}
\def\HHmpdual{{{\Hil}_{1/w}^q}}
\def\HHmpdddd{{\left( \HHmp \right)'}}
\def\HHmi{{{\Hil}_w^\infty}}
\def\HHmidual{{{\Hil}_{1/w}^1}}
\def\HHmidddd{{\left( \HHmi \right)'}}
\def\Hn{\Hil^{00}}

\def\HHmptens{{}_{\otimes} \Hil_{W}^{p_1,p_2}}


\newcommand{\range}[1]{\mathsf{ran}\left( #1 \right)} %sf rm tt
\newcommand{\domain}[1]{\mathsf{dom}\left( #1 \right)} %sf rm tt
\newcommand{\support}[1]{\mathsf{supp}\left( #1 \right)} %sf rm tt
\newcommand{\identity}[1]{\mathsf{id}_{ #1 }}
\newcommand{\kernel}[1]{\mathsf{ker}\left( #1 \right)}
\newcommand{\trace}[1]{\mathsf{tr}\left( #1 \right)}
\newcommand{\finspan}[1]{\mathsf{span}\left( #1 \right)}
\newcommand{\clspan}[1]{\overline{\finspan{#1}}}

\newcommand{\kernelc}[1]{\mathsf{ker^c}\left( #1 \right)}
\newcommand{\rangec}[1]{\mathsf{ran^c}\left( #1 \right)} %sf rm tt



\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\esssup}{ess\,sup}
\DeclareMathOperator{\essinf}{ess\,inf}


\unitlength1mm


\definecolor{darkviolet}{rgb}{0.58,0,0.83} %{148,0,211}
\def\xxl{\color{darkviolet}}
\def\xxlnew{\color{red}}

\newcommand{\C}{{\mathcal{C}o_\pi}\,}
\newcommand{\CiP}[1]{{\mathcal{C}o_{\pi_1}L^{#1}_{1/w_1}(G_1)}\,}
\newcommand{\CiiP}[1]{{\mathcal{C}o_{\pi_2}L^{#1}_{1/w_2}(G_2)}\,}
\newcommand{\Ci}[1]{{\mathcal{C}o_{\pi_1}L^{#1}_{w_1}(G_1)}\,}
\newcommand{\Cii}[1]{{\mathcal{C}o_{\pi_2}L^{#1}_{w_2}(G_2)}\,}
\newcommand{\CiiN}[1]{{\mathcal{C}o_{\pi_2}L^{#1}(G_2)}\,}
\newcommand{\CiN}[1]{{\mathcal{C}o_{\pi_1}L^{#1}(G_1)}\,}
\newcommand{\Cim}[1]{{\mathcal{C}o_{\pi_1}L^{#1}_{m_1}(G_1)}\,}
\newcommand{\Ciim}[1]{{\mathcal{C}o_{\pi_2}L^{#1}_{m_2}(G_2)}\,}
\newcommand{\pio}{\pi_\otimes}

\newcommand{\sd}[3]{#1^{\left(#3,#2\right)}}
\newcommand{\ds}[3]{#1^{\overline{\left( #3,#2\right)}}}
\newcommand{\sda}[3]{#1^{\left({#3}^*,#2\right)}}
\newcommand{\dsa}[3]{#1^{\overline{\left( {#3}^*,#2\right)}}}

\def\Phisd{\sd{\Phi}{\Psi}{U}}
\def\phisd{\sd{\phi}{\psi}{U}}

\def\Psipd{\ds{\Psi}{\Phi}{U}}
\def\psipd{\ds{\psi}{\phi}{U}}



==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


